Learning vs Retrieval: The Role of In-Context Examples in Regression with Large Language Models

Generative Large Language Models (LLMs) are capable of being in-context learners. However, the underlying mechanism of in-context learning (ICL) is still a major research question, and experimental research results about how models exploit ICL are not always consistent. In this work, we propose a framework for evaluating in-context learning mechanisms, which we claim are a combination of retrieving internal knowledge and learning from in-context examples by focusing on regression tasks. First, we show that LLMs can solve real-world regression problems and then design experiments to measure the extent to which the LLM retrieves its internal knowledge versus learning from in-context examples. We argue that this process lies on a spectrum between these two extremes. We provide an in-depth analysis of the degrees to which these mechanisms are triggered depending on various factors, such as prior knowledge about the tasks and the type and richness of the information provided by the in-context examples. We employ three LLMs and utilize multiple datasets to corroborate the robustness of our findings. Our results shed light on how to engineer prompts to leverage meta-learning from in-context examples and foster knowledge retrieval depending on the problem being addressed.

==> Chapters/checklist.tex <==
\section{Reproducibility Checklist}

\subsubsection{This paper:}

\begin{itemize}

\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{yes}/partial/no/NA): Prompt Configurations section and Models and Metrics section.
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textbf{yes}/no)
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textbf{yes}/no): Introduction section and Appendix A.
\end{itemize}

\subsubsection{Does this paper} make theoretical contributions? (yes/\textbf{no})

If yes, please complete the list below.

\begin{itemize}
\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
\item Proofs of all novel claims are included. (yes/partial/no)
\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\subsubsection{Does this paper} rely on one or more datasets? (\textbf{yes}/no)

If yes, please complete the list below.
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets (\textbf{yes}/partial/no/NA): Datasets section.
\item All novel datasets introduced in this paper are included in a data appendix. (\textbf{yes}/partial/no/NA): datasets are attached and Section A explains the datasets in multiple subsections.
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/\textbf{NA})
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textbf{yes}/no/NA)
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textbf{yes}/partial/no/NA)
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/\textbf{NA})
\end{itemize}

\subsubsection{Does this paper} include computational experiments? (\textbf{yes}/no)

If yes, please complete the list below.

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (\textbf{yes}/partial/no).
\item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{yes}/partial/no)
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{yes}/partial/no)
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textbf{yes}/partial/no)
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/\textbf{NA})
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textbf{yes}/partial/no) Appendix C
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{yes}/partial/no): Models and Metrics.
\item This paper states the number of algorithm runs used to compute each reported result. (\textbf{yes}/no)
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{yes}/no)
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\textbf{yes}/partial/no)
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\textbf{yes}/partial/no/NA) Appendix C
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{yes}/partial/no/NA) Appendix C

\end{itemize}

==> Chapters/old_june_Introduction.tex <==

\section{Introduction}

% Intro
The emergence of transformers~\cite{NIPS2017_3f5ee243} has revolutionized natural language processing, leading to the development of LLMs such as GPTs~\cite{brown2020languagemodelsfewshotlearners} and LLaMA~\cite{touvron2023llamaopenefficientfoundation}. In addition to their impressive zero-shot performance, these models demonstrated a surprising capability by learning a task from a few examples, called in-context learning (ICL)~\cite{brown2020languagemodelsfewshotlearners}. In tasks where both zero-shot and ICL settings are applicable, ICL consistently outperforms the zero-shot setting~\cite{brown2020languagemodelsfewshotlearners,liu-etal-2022-makes}. However, the inner mechanism of the LLMs and their utilization of the provided ICL information remains a mystery. 

%Previous context
    %ICL helps finding the line of reasoning by COT
   % Different way that ICL helps: internal mechanism, why it works. 
% Few-shot , COT, ...  
%\pk{if you want to explain various forms of ICL, start with few-shot }
In its simple form, ICL, requires a few examples (typically 2-5 but sometimes in very large numbers) of the raw unedited input and output which causes learning from these input-output pairs. This simple form of ICL alone, improves the accuracy of many tasks significantly such as NLI~\cite{brown2020languagemodelsfewshotlearners} by just demonstrating a few examples. Subsequently, others tried to utilize the few-shot example in more sophisticated ways such as providing the templates of the required reasoning, often in a step-by-step manner, referred to as Chain of Thought (COT)~\cite{wei2023chainofthoughtpromptingelicitsreasoning}. COT emphasizes following the instructed line of reasoning to find the solution rather than learning from the few provided examples, resulting in improved accuracy over simple ICL. However, COT is not universally helpful. As the research results show COT does not provide any benefits in tasks where the reasoning is simple, such as in GSM8K dataset~\cite{cobbe2021trainingverifierssolvemath}. \cite{Min2022RethinkingTR} goes a step further and argues that the ground truth values in the ICL are irrelevant and do not affect the accuracy. It goes as far as claiming that replacing the ground truth values with random labels,  barely hurts the performance with consistent results in 12 tested models on a wide range of tasks. They claim the only important aspects of ICL exclusively are defining label space, input distribution, and the general format of the task. These results invalidate the hypothesis of LLMs being meta-learners that learn to learn from in-context examples. 

% from here you talk about the underlying mechanism. 
    %ICL can foster meta-learning and regression
On the other hand, another prevalent hypothesis suggests that transformers are effective meta-learners, and LLMs can generate accurate predictions based solely on numerical input and output values. \cite{bai2023transformers,Garg2022WhatCT} theoretically proves and practically tests that an encoder-based transformer is capable of implementing generalized linear models such as Ridge and Lasso, in-context. While their setting is controlled and their data is artificial, they argue that their findings can extend to decoder-based transformers such as LLMs. \cite{Garg2022WhatCT} expands on this work by directly using a decoder-based model, a modified GPT2 architecture that inputs features inside embedding (instead of tokens) and outputs a number as the regression answer. They conclude that this model surpasses models such as a 2-layer Multi-Layer Perceptron (MLP) and a decision tree by meta-learning. Further, \cite{vacareanu2024words} directly uses LLMs to test the regression capabilities within settings such as limited data instances and a limited number of features. It concludes that LLMs are capable regressors and in some cases, they outperform traditional models such as linear regression and MLP. However, according to our findings in this paper, the claim of avoiding data contamination is not well-supported. %is weak and in contrast to our findings.


% grouth truth doesnt matter


\begin{figure*}[h]
    \centering
    \includegraphics[width=0.86\textwidth]{introv2}
    \caption{The three main prompt configurations that we use in our regression task. In configuration a) the actual names of the features and the output are known and the LLM is asked to guess the ``Price'' of a used car based on features. Configuration b) is similar to a) except that we the real names of the features are anonymized. Here, the LLM is asked to estimate the ``Output''. Finally, in Configuration c), we replace the real prices of in-context examples with randomly generated numbers.} 
    \label{fig:intro}
\end{figure*}

%The findings of research around transformers and their meta-learning directly contrast the findings of previously mentioned \cite{Min2022RethinkingTR} which argued that labels are not relevant in learning. \pk{is this contradictory?} 

To analyze the source of the inconsistency of the previous research results on ICL capabilities, we propose an evaluation framework. In this regard, we conduct a comparative study of different LLMs and datasets, focusing specifically on simple regression problems as our testing ground. In our evaluation framework, we query the LLM to estimate an output number based on a set of (feature, value) pairs as shown in Figure~\ref{fig:intro} given ICL examples. We opted for regression tasks primarily for two reasons. First, this choice aligns our work with the majority of related research discussed earlier, facilitating direct comparisons and building upon existing findings. This task also has a continues output space which is challenging for an LLM specially when no ICL examples are provided (as our LLM baseline to compare to ICL). We show that LLMs can perform regression on realistic datasets and measure the extent to which the LLM retrieves its internal knowledge versus learning from in-context examples. We argue that this process lies on a spectrum between these two extremes. We provide an in-depth analysis of the degrees to which these mechanisms are triggered depending on the factors that we use in our framework: the number of (feature, value) pairs, the number of in-context examples, and the configurations of our prompting strategies.

As our contributions, we answer the following questions:
\begin{enumerate}


\item  Can LLMs learn from regression examples of \textbf{realistic} datasets in context?

%\item  How do LLMs  utilize various types of information in ICL? too repeating

\item  How does the internal knowledge of LLMs impact their utilization of ICL information for retrieval vs learning?

\item How does the type of information in ICL guide LLMs in utilizing ICL information for retrieval vs learning?

\item  How can we improve prompt engineering for a specific task and LLM by controlling internal knowledge retrieval vs learning in context?

\item  How to disentangle internal knowledge vs data contamination in regression tasks? \pk{do you answer this?} \darius{last point of disscusions}

\end{enumerate}





==> Chapters/titles.tex <==
Learning vs Retrieval: The Role of In-Context Examples in Regression with LLMs

Learning from vs. Retrieving with In-Context Examples in Large Language Models"

Learning from In-Context Examples vs. Retrieving Internal Knowledge for Regression in LLMs

